VideoScore: Building Automatic Metrics to Simulate Fine-grained Human Feedback for Video Generation

The recent years have witnessed great advances in video generation. However, the development of automatic video metrics is lagging significantly behind. None of the existing metric is able to provide reliable scores over generated videos. The main barrier is the lack of large-scale human-annotated dataset. In this paper, we release VideoFeedback, the first large-scale dataset containing human-provided multi-aspect score over 37.6K synthesized videos from 11 existing video generative models. We train VideoScore (initialized from Mantis) based on VideoFeedback to enable automatic video quality assessment. Experiments show that the Spearman correlation between VideoScore and humans can reach 77.1 on VideoFeedback-test, beating the prior best metrics by about 50 points. Further result on other held-out EvalCrafter, GenAI-Bench, and VBench show that VideoScore has consistently much higher correlation with human judges than other metrics. Due to these results, we believe VideoScore can serve as a great proxy for human raters to (1) rate different video models to track progress (2) simulate fine-grained human feedback in Reinforcement Learning with Human Feedback (RLHF) to improve current video generation models.

==> tables/abilities.tex <==
% \begin{wraptable}{r}{0.7\textwidth}
\definecolor{darkgreen}{rgb}{0.0, 0.8, 0.0}
\definecolor{darkred}{rgb}{0.8, 0.0, 0.0}
\begin{table}[!h]
\centering
\vspace{-2em}
\small
\def\arraystretch{1.0}
\setlength\tabcolsep{2 pt}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Platform}  & \textbf{\begin{tabular}[c]{@{}c@{}}Text-To-Image\\ Generation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Text-Guided\\ Image Editing\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Text-To-Video\\ Generation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Human Label\\ Transparency\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} Open/Public \\ Voting Process\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} Judging \\ MLLM judge\end{tabular}} \\
\midrule
T2I-CompBench~\cite{huang2023t2icompbench} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} \\ 
HEIM~\cite{lee2024holistic} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}}  \\ 
ImagenHub~\cite{ku2024imagenhub} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}}\\ 
VBench~\cite{huang2023vbench} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}}\\ 
EvalCrafter~\cite{liu2023evalcrafter} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} \\ 
\midrule
\textbf{\arena} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}}\\ 
\bottomrule
\end{tabular}}
\caption{Comparison with different evaluation platforms on different properties.}
\label{tab:baselines}
\end{table}
% \end{wraptable}

==> tables/feature_based_score.tex <==

\begin{table*}[!ht]

\small
\centering
\begin{tabular}{c|c|c}
\toprule
Dimenson & Metric Name & Implementation    \\
\midrule
Visual Qualituy  & PIQE &                          
    $ \frac{1}{N} \sum^{N}_{i=1} PIQE(f_i)$   \\
\midrule
Visual Qualituy & BRISQUE  & $ \frac{1}{N} \sum^{N}_{i=1} BRISQUE(f_i)$  \\
\midrule
Temporal Consistency & CLIP-sim & $ \frac{1}{N-1} \sum^{N-1}_{i=1} cos(CLIP(f_i),CLIP(f_{i+1}))$  \\
\midrule
Temporal Consistency & DINO-sim & $ \frac{1}{N-1} \sum^{N-1}_{i=1} cos(DINO(f_i),DINO(f_{i+1}))$  \\
\midrule
Temporal Consistency & SSIM-sim & $ \frac{1}{N-1} \sum^{N-1}_{i=1} SSIM(f_i,f_{i+1})$  \\
\midrule
Dynamic Degree & MSE-dyn & $ \frac{1}{T-1} \sum^{T-1}_{i=1} MSE(f_i,f_{i+1})$  \\
\midrule
Dyanmic Degree & SSIM-dyn & $ \frac{1}{T-1} \sum^{T-1}_{i=1} SSIM(f_i,f_{i+1})$  \\
\midrule
Text-to-Video Alignment & CLIP-Score & $ \frac{1}{N} \sum^{N}_{i=1} cos(CLIP(f_i),CLIP(prompt)$  \\
\midrule
Text-to-Video Alignment & X-CLIP-Score & $ cos(XCLIP(video), XCLIP(prompt))$  \\
\bottomrule
\end{tabular}
\caption{Feature based scores}
\label{tab:feature_based_score}
\end{table*}

==> tables/test_genaibench.tex <==
\begin{table*}[!ht]
\caption{Pairwise preference accuracy of \score on GenAI-Bench test set}
\label{tab:test_genaibench}
\small
\centering
\begin{tabular}{ccccccc}
\toprule
Method                  & Visual               & Temporal             & Dyanmic              & Text Align           & Facutal              & Overall              \\
\midrule
Random                  & 37.7                 & 37.7                 & 37.7                 & 37.7                 & 37.7                 & 37.7                 \\
\midrule
\multicolumn{7}{c}{\textbf{Feature-basd Automatic Metrics}}                                                                                                       \\
\midrule
PIQE                    & 34.1                 & 34.1                 & 34.1                 & 34.1                 & 34.1                 & 34.5                 \\
BRISQUE                 & 38.5                 & 38.5                 & 38.5                 & 38.5                 & 38.5                 & 38.5                 \\
CLIP-sim                & 34.1                 & 34.1                 & 34.1                 & 34.1                 & 34.1                 & 34.1                 \\
DINO-sim                & 31.4                 & 31.4                 & 31.4                 & 31.4                 & 31.4                 & 31.4                 \\
SSIM inter-frame        & 28.4                 & 28.4                 & 28.4                 & 28.4                 & 28.4                 & 28.4                 \\
SSIM for dynamic degree & 38.5                 & 38.5                 & 38.5                 & 38.5                 & 38.5                 & 38.5                 \\
MSE for dynamic degree  & 34.2                 & 34.2                 & 34.2                 & 34.2                 & 34.2                 & 34.2                 \\
CLIP-Score              & 45.0                 & 45.0                 & 45.0                 & 45.0                 & 45.0                 & 45.0                 \\
X-CLIP-Score            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\midrule
\multicolumn{7}{c}{\textbf{MLLM Prompting}}                                                                                                                       \\
\midrule
LLaVA-1.5-7B            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
LLaVA-1.6-7B            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
Idefics2                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
Gemini-1.5-Flash        & 38.35                & 36.2                 & 33.4                 & 43.87                & 46.77                & 67.07                \\
Gemini-1.5-Pro          & 41.07                & 35.64                & 30.87                & 43.22                & 43.31                & 60.9                 \\
GPT-4o                  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\midrule
\multicolumn{7}{c}{\textbf{Ours}}                                                                                                                                 \\
\midrule
\score (gen)            & 37.7                 & 35.2                 & 35.9                 & 34.6                 & 37.7                 & 59.0                 \\
\score (reg)            & \textbf{63.1}        & \textbf{72.4}        & \textbf{64.6}        & \textbf{76.0}        & \textbf{71.8}        & \textbf{78.5}        \\
\rowcolor{LightCyan} $\Delta$ over Best Baseline & 18.1                 & 27.4                 & 19.6                 & 31.0                 & 25.0                 & 11.4          \\
\bottomrule
\end{tabular}
\end{table*}

==> trash/ablation_ec.tex <==
\begin{table*}[!ht]
  \caption{Correlation (Spearman's $\rho$ ) between model answer and human reference on our EvalCrafter Benchmark}
  \label{tab:abl_ec}
  \small
  \centering
\begin{tabular}{lccc}
\toprule
& Visual Quality              & Temporal Consistency                   & Text Alignment                 \\ 
\midrule
\multicolumn{4}{c}{\textbf{Baseline}} \\
\midrule
Random Guess  & \multicolumn{1}{r}{-2.0} & \multicolumn{1}{r}{1.4} & \multicolumn{1}{r}{-0.9} \\
all good & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} \\ 
\midrule
\multicolumn{4}{c}{\textbf{Ours}} \\
\midrule
\score (reg)            & \multicolumn{1}{r}{-14.1} & \multicolumn{1}{r}{3.4} & \multicolumn{1}{r}{15.1} \\
\score (gen)             & \multicolumn{1}{r}{6.7}  & \multicolumn{1}{r}{15.4} & \multicolumn{1}{r}{9.0} \\
idefics2-reg                    &                             &                            &                            \\
idefics2-gen                    &                             &                            &                            \\
videollava-gen                  & \multicolumn{1}{r}{9.9}  & \multicolumn{1}{r}{12.9} & \multicolumn{1}{r}{6.5} \\
mantis-idefics2-33k-regression (anno only) 
& \multicolumn{1}{r}{42.4 }  & \multicolumn{1}{r}{51.3} & \multicolumn{1}{r}{59.5} \\

mantis-idefics2-33k-generation (anno only) & \multicolumn{1}{r}{20.8}  & \multicolumn{1}{r}{51.3} & \multicolumn{1}{r}{10.7} \\ 
\bottomrule
\end{tabular}
\end{table*}

==> trash/ablation_our_bench.tex <==
\begin{table*}[!ht]
  \caption{Correlation (Spearman's $\rho$ ) between model answer and human reference on our test benchmark}
  \label{tab:abl_our_bench}
  \small
  \centering
\begin{tabular}{lccccc}
\toprule
Method                                & Visual      & Temporal        & Dynamic            & Text Align       & Factual        \\ 
idefics2-43k-regression               &             &                 &                    &                  &                  \\
idefics2-43k-generation               & 0.8423      & 0.7606          & 0.7219             & 0.5344           & 0.7756           \\
videollava-43k-generation             & 0.8254      & 0.7356          & 0.6934             & 0.5992           & 0.7510           \\
mantis-idefics2-33k-regression (anno only)      & 0.5212    & 0.4635  & 0.4041             & 0.2094           & 0.4510           \\
mantis-idefics2-33k-generation (anno only)      & 0.6151 & 0.4190 & 0.3770 & 0.4761 & 0.5097  \\
\bottomrule
\end{tabular}
\end{table*}
